Counterfactual Explanations for Graph Classification Through the Lenses of Density

Counterfactual examples have emerged as an effective approach to produce simple and understandable post-hoc explanations. In the context of graph classification, previous work has focused on generating counterfactual explanations by manipulating the most elementary units of a graph, i.e., removing an existing edge, or adding a non-existing one. In this paper, we claim that such language of explanation might be too fine-grained, and turn our attention to some of the main characterizing features of real-world complex networks, such as the tendency to close triangles, the existence of recurring motifs, and the organization into dense modules. We thus define a general density-based counterfactual search framework to generate instance-level counterfactual explanations for graph classifiers, which can be instantiated with different notions of dense substructures. In particular, we show two specific instantiations of this general framework: a method that searches for counterfactual graphs by opening or closing triangles, and a method driven by maximal cliques. We also discuss how the general method can be instantiated to exploit any other notion of dense substructures, including, for instance, a given taxonomy of nodes. We evaluate the effectiveness of our approaches in 7 brain network datasets and compare the counterfactual statements generated according to several widely-used metrics. Results confirm that adopting a semantic-relevant unit of change like density is essential to define versatile and interpretable counterfactual explanation methods.

==> sections/1intro_old.tex <==
\section{Introduction}\label{sec:intro}
Many applications, such as time series forecasting, text classification, and speech recognition, have benefited greatly from the effectiveness of AI systems. However, as these systems become more complex, users may find it challenging to understand their output.
This opacity can lead to uninformed decisions, complicate the audit process, and impede trust in AI adoption.
One solution is to use only interpretable models (white-box), such as linear and logistic regression, decision trees, and Lasso and Ridge regressions \cite{rudin2019stop}. These models are easier for humans to comprehend as they are transparent and their inner workings can be interpreted.
Alternatively, post-hoc explanation methods can be employed to make black-box models more interpretable \cite{biran2017explanation,guidotti2018survey}.
Explanations of black-box models can help to build trust in AI systems by enabling users to understand the decision-making process and assess the reliability of the system.
This is particularly important in applications that impact people's lives, such as healthcare, finance, and criminal justice~\cite{bhatore2020machine,kononenko2001machine}.
%However, one drawback of these models is that they are often complex and difficult to interpret. This means that users, developers, and in general stakeholder may struggle to understand why a particular decision was made or suggested. Given that these AI tools provide significant support in highstake decision making processes supporting humans, providing understandable explanations for the outputs made by machine learning models has become a critical task for their application in sensitive field such as finance, credit scoring, and healthcare.

%check for a better definition
\textit{Counterfactual explanations}~\cite{moraffah2020causal} are a method of explaining predictions for individual examples. 
These explanations take the form of "If X had been different, Y would not have occurred", making them concise and easy to understand.
A counterfactual explanation consists in a \textit{counterfactual example}, which is a modified version of the instance that leads to a different outcome of the black-box model.
Counterfactual explanations have been increasingly used in recourse generation for loan applications~\cite{karimi2020survey}, among others. 
An example of counterfactual explanation for a person $P$ with a credit score of $400$ who applied for a loan and was rejected is as follows: 
\begin{displayquote}
\textit{If the credit score of $P$ had been 700, $P$ would have qualified for the loan.}
\end{displayquote}
% Therefore, the counterfactual explanation is made selecting a counterfactual instance and then the difference between the original and the counterfactual instance is highlighted in the counterfactual statement.

% advantages of counterfactual as explanations
Define and generate an optimal counterfactual is not a straightforward task, because counterfactual examples must be searched in a huge feature space, where some states may not be feasible. As an example, the following counterfactual example for a woman $P$ whose college application got rejected is not feasible:
\begin{displayquote}
\textit{If $P$ were a man, she would have been admitted to college.}
\end{displayquote}

Due to these challenges, there are multiple approaches to retrieve counterfactuals, such as with optimization strategies, heuristics search, and decision trees~\cite{guidotti2022counterfactual}. 
% ---------

Various metrics have been proposed to evaluate a counterfactual instance. 
\textbf{Fidelity} tells whether the prediction for the counterfactual instance is different from the prediction for the original example; 
\textbf{Similarity} measures how similar is the counterfactual instance to the original example;
\textbf{Sparsity} measures the proportion of features changed to generate the counterfactual instance; 
\textbf{Feasibility} indicates whether the counterfactual instance is feasible or not;
\textbf{Efficiency} determines how fast the search for the counterfactual instance is;
and \textbf{Diversity} measures the level of diversity of a set of counterfactual explanations generated for the same example. By providing a set of diverse explanations, the intricate details of the black-box model can be brought to light~\cite{mothilal2020explaining}.

In this paper, we emphasize the significance of \textbf{semantic} in generating diverse counterfactual explanations for \textit{graph data}, and show how it can improve the comprehensibility of the explanations while also distinguishing them from adversarial attacks~\cite{browne2020semantics}.
% The term semantic is used ambiguously in Machine Learning and Deep Learning \cite{bengio2009learning,lecun2015deep}.
% We refer to semantics as the human-understandable logic that is used to connect sign and signified \cite{browne2020semantics}. 
In the field of counterfactual-based explainable AI, semantic is defined as the unit of change between the original instance and its counterfactual counterpart.
An instance of how semantic is critical in counterfactual search can be seen in the domain of  Computer Vision, where semantics helps to discern a counterfactual explanation from an adversarial attack~\cite{akula2020cocox}. 
Let assume that the black-box model is an image classifier and that the input instance is a horse miss-classified as a zebra.
with a low-level semantic such as pixel color, the counterfactual explanation would be useless, unless as an adversarial attack. 
With a human-understandable concept as semantic, such as stripes, the counterfactual would be easily interpreted by a human.
% Check!!!!
%Furthermore, we show that the semantic of \textit{Counterfactual Statements} can be encoded in the heuristic search method and measured by the distance between the original and the counterfactual graphs.
\subsection{Semantic-based Counterfactuals for Brain Networks}
\begin{figure}[t!]
	\begin{minipage}[b]{0.49\textwidth}
    	%\centering
    	\includegraphics[width=\textwidth]{Figures/10.png}
   \end{minipage}
   \hfill
   \begin{minipage}[b]{0.49\textwidth}
    	%\centering
    	\includegraphics[width=\textwidth]{Figures/10_heatmap.png}
   \end{minipage}
   \caption{On the right: brain network with nodes colored according to the AAL atlas, and regions changed in its counterfactual instance; blue edges denote dense regions added to the counterfactual graph, while red edges denote dense regions removed. On the left: number of intra- and inter-region edges involved in the counterfactual generation; the low diagonal matrix concerns the edges removed, and the upper diagonal matrix concerns the edges added.}
   \label{fig:first_fig}
\end{figure}

We consider binary classifiers $f:\mathcal{G} \rightarrow \{0,1\}$ for graphs $G$. 
% Given a classifier $f:\mathcal{G} \rightarrow \{0,1\}$, a \textbf{counterfactual graph} $G'$ for a $G \in \mathcal{G}$ is a graph $G' \in \mathcal{G}$ that is classified in the opposite class, i.e., $f(G')=1-f(G)$, with the minimum change between the two graphs, and possibly satisfies some other criteria~\cite{Dandl_2020}.
Previous works~\cite{countg} generate counterfactual graphs by applying the finest possible change to the input graph, i.e., edge addition/deletion.
Then, they evaluate the goodness of the counterfactual graphs found in terms of the symmetric difference between the two edge sets. 
In some applications \cite{lanciano2023survey}, however, an edge-based semantic may lead to counterfactual graphs less relevant than those obtained by simultaneously changing multiple edges in specific parts of the graph.
We present a novel approach for constructing \textbf{density-based counterfactual graphs} that leverages a new semantic based on density. 
In detail, this approach identifies the most informative regions of the graphs and manipulates their density.
%We hypothesize that this method will enhance the accuracy and interpretability of the counterfactual graphs by focusing on the aspects of the data that are most likely to impact the outcomes of interest.
An instance of the practical utilization of density-based counterfactual graph search is evident in the classification of brain networks.
Brain networks can be modeled as undirected graphs, with nodes denoting Regions of Interest (ROIs), and edges indicating correlations of activation.
%Figure \ref{fig:first_fig}, for instance, shows the brain parcellation given by the AAL atlas~\cite{aal}: different node colors indicate different relevant areas of the brain.
%In this scenario, explaining the outcome with density-based counterfactual graph can be more descriptive than using changes at edge level, because it uses a semantic of explanation that is consistent with the language used to describe the organization of the brain.

% \begin{comment}
% \begin{figure}[t!]
%     \centering
%     \includegraphics[width=\linewidth]{Figures/10.png}
%     \vspace{-4mm}
%     \caption{A brain network with nodes colored according to the AAL atlas, and regions involved in the generation of its counterfactual graph: blue edges denote the dense region to add to the counterfactual graph, red edges denote the dense region to remove, and gray edges indicate edges not relevant for the generation process.}
%     \label{fig:brain_example}
% \end{figure}

% \begin{figure}[t!]
%     \centering
%     \includegraphics[width=\linewidth]{Figures/10_heatmap.png}
%     \vspace{-4mm}
%     \caption{Distribution across different regions in the brain parcellation of the edges involved in the counterfactual generation: the low diagonal matrix concerns the edges removed, while the upper diagonal matrix concerns the edges added.}
%     \label{fig:brain_example_heat}
% \end{figure}
% \end{comment}
RoIs are usually grouped into distinct partitions (\emph{brain parcellation}), according to several properties such as structural and functional markers.
Figure~\ref{fig:first_fig} shows a brain taken from the Autism Brain Image Data Exchange (ABIDE) dataset~\cite{craddock2013neuro}. Nodes in different brain parcellations are denoted with different colors.
% The brain in figure \ref{fig:first_fig} is part of a brain dataset about patients with Autism Spectrum Disorder (ASD) and Typically Developed (TD) patients.
In this context, explaining the outcome of the classifier through the use of density-based counterfactual graph explanations can be more comprehensive than changes made at the edge level. This is due to the fact that the semantic employed in such explanations is more consistent with the terminology used to describe the organization of the brain.
As an example, given the brain in Figure~\ref{fig:first_fig}, our density-based counterfactual method finds a counterfactual graph by removing the dense region colored in red and adding the dense region colored in blue.
Such result can be formulated in the form of a counterfactual statement as follows:
\begin{displayquote}
\textit{Patient X is classified as Typically Developed. If X's brain had less co-activation between the \textit{Temporal Lobe} and the \textit{Parietal Lobe}, and more co-activation between the \textit{Frontal Lobe} and the \textit{Cerebellum}; then X would have been classified as Autism Spectrum Disorder.}
\end{displayquote}
The change in density in the counterfactual graph for $X$ is shown in the matrix in Figure~\ref{fig:first_fig} (right).
This matrix illustrates the number of edges added/removed within and between different regions in the brain parcellation.

In the next sections, we formalize the \textit{density-based counterfactual} problem, discuss the intuition behind such formalization, propose a clique-based framework for searching counterfactual graphs, and present some experimental results.
\mynote[from=Giulia]{Add description of the methods and main results.}

==> sections/5.2syntetic.tex <==
\subsection{Validation of \dcs}
% \mynote[from=Carlo]{there are a multiple synthetic datasets that are used as benchmarks, maybe it's better to use them instead of ours?}
%Synthetic data Generation and results
We validate {\dcs} in two synthetic datasets equipped with a white-box binary classifier.
The graph generation process takes in input a set of nodes $V$ and a number of graphs $N$.
The set of nodes is partitioned into two subsets $S_0$ and $S_1$ of equal size, and then, for each class $i \in \{0, 1\}$, $N/2$ graphs are generated according to the following procedure:
\textbf{(i)} select one (1SG) or two (2SG) subgroups of nodes in $SG \subseteq S_i$, 
\textbf{(ii)} build $c$ random cliques among nodes within the same subgroup,
\textbf{(iii)} apply a Barabási–Albert preferential attachment algorithm \cite{albert2002statistical} with parameters $m$, $p$, and $q$, to add structure within $S_{1-i}$ and between $S_i$ and $S_{1-i}$
\footnote{We set $N_{1SG} = 100$ and $N_{1SG} = 200$; $SG_{1SG} = 1/4 \cdot |V|$ and $SG_{2SG} = 1/8 \cdot |V|$; $c_{1SG} = 10$ and $c_{2SG} = 20$; $m = SG$, $p = 5$ and $q = 0.7$.}.

This way, for each $i$, we obtain graphs with dense regions in $S_i$, but sparse in $S_{1-i}$.
\ref{fig:synt} illustrates the dense regions in the graphs for each class, in terms of triangle count at node level. The upper chart shows the average triangle count for the synthetic dataset 1SG, while the lower chart shows the same quantity for 2SG.

\begin{figure}[thb]
    \begin{minipage}[b]{0.49\textwidth}
    \centering
    \includegraphics[width=\textwidth]{Figures/tri__v2.2.png}
   \end{minipage}
   \hfill
   \begin{minipage}[b]{0.49\textwidth}
    \centering
    \includegraphics[width=\textwidth]{Figures/tri__b6.png}
   \end{minipage}
   \caption{Average triangle count at node level, for synthetic graphs in the same class, in 1SG (upper) and 2SG (lower).}
   \label{fig:synt}
\end{figure}

Then, we build a white-box classifier using the same logic of the graph generation process, to achieve perfect accuracy.
\mynote[from=Carlo]{Is it fine to use this very simple white box classifier? Is it better to train a black-box model?}
%Explain in the appendix the classifier algorithm

\begin{table}[thb]
	\centering
	\caption{Quartiles of symmetric difference (percentage) $d_{\%}$, and number of iterations $I$, for the synthetic datasets 1SG and 2SG.}
	\label{tab1}
	\begin{tabular}{ccrrrrr}
		\toprule
		\textbf{Dataset} &  \textbf{Measure} & \textbf{Q0} & \textbf{Q1} & \textbf{Q2} & \textbf{Q3} & \textbf{Q4} \\ 
		\midrule
		\multirow{2}{*}{1SG} 
		& $d_{\%}$ & 18.5 & 39.3 & 55.5 & 80 & 100 \\
		%& $d_{cl}$ & 0.5 & 0.65 & 0.7 & 0.77 & 0.92 \\
		% & Cl. sort & -2.01 & 0.14 & 0.38 & 0.51 & 0.71 \\
		& $I$ & 1 & 2 & 3 & 6 & 21 \\
      \hline
		\multirow{2}{*}{2SG} 
		& $d_{\%}$ & 42.1 & 81.6 & 100 & 100 & 100 \\
		%& $d_{cl}$ & 0.43 & 0.52 & 0.57 & 0.61 & 0.73 \\
		% & Cl. sort & -3.52 & -1.33 & -0.35 & 0.3 & 0.68 \\
		& $I$ & 2 & 3 & 6 & 9 & 19 \\
		\bottomrule
	\end{tabular}
\end{table}

\ref{tab1} summarizes the results of the validation of \dcs.
In details, it reports the quartiles of the symmetric differences (percentage of edges modified) $d_{\%}$, the closeness $d_{cl}$ between the original and the counterfactual graphs, and the number of iterations $I$, for both 1SG and 2SG.
The flip rate is $100\%$ in both datasets. 
However, the symmetric difference $d_{\%}$ is quite high, especially in the 2SG dataset, where in more that half of the cases of the edges are changed.

\ref{fig:hm_bi} illustrates the evolution of the dense regions in one graph from the 2SG dataset at each iteration of \dcs.


\begin{figure}[thb]
 \vspace{-2mm}
    \centering
    \includegraphics[width=\linewidth]{Figures/ev_tri_p__b6.png}
    \vspace{-8mm}
    \caption{Evolution of number of triangles for each node. Even indexes represents empty search sub-step, and odd indexes fill search sub-step. Each column is the difference between the graph at the iteration (i-1) and the graph at the current iteration (i) of the number of triangle score at node level.}
    \label{fig:hm_bi}
    \vspace{-2mm}
\end{figure}

\mynote[from=Giulia]{Elaborate on the results in \ref{tab1} and \ref{fig:hm_bi}.}


\begin{table*}[thb]
	\centering
	\footnotesize
	\caption{}
	\label{tab:iterations}
	\begin{tabular}{c c c ccccc}
		\toprule
		&  &  & \multicolumn{5}{c}{Iterations} \\
	   \cmidrule(lr){4-8}
	   \textbf{Data} & 		
	   \textbf{Type} & 		
	   \textbf{FR0/FR1} & 
	   \textbf{min} & \textbf{25-p} & \textbf{50-p} & \textbf{75p} & \textbf{max} \\
    \midrule
AUT & EDG & 100.0/84.8 & 1 & 24.0 & 40.0 & 57.25 & 2000 \\
AUT & DAT+BW & 100.0/100.0 & 79 & 129.0 & 149.0 & 168.0 & 313 \\
AUT & TRI & 100.0/100.0 & 1 & 9.0 & 22.0 & 52.0 & 610 \\
AUT & CLI & 90.9/100.0 & 2 & 2.0 & 3.0 & 17.0 & 60 \\
AUT & RCLI & 96.4/93.5 & 3 & 6.0 & 11.0 & 83.0 & 671 \\
AUT & DAT & 100.0/100.0 & 102 & 102.0 & 102.0 & 102.0 & 102 \\
  \hline
BIP & EDG & 70.0/100.0 & 1 & 9.0 & 25.0 & 51.0 & 2000 \\
BIP & DAT+BW & 100.0/100.0 & 61 & 127.0 & 201.5 & 384.5 & 1477 \\
BIP & TRI & 100.0/100.0 & 1 & 1.0 & 6.0 & 25.0 & 595 \\
BIP & CLI & 100.0/100.0 & 2 & 2.0 & 6.5 & 8.75 & 20 \\
BIP & RCLI & 94.0/100.0 & 3 & 10.0 & 153.0 & 257.0 & 675 \\
BIP & DAT & 100.0/100.0 & 119 & 119.0 & 119.0 & 119.0 & 119 \\
  \hline
ADHD & EDG & 75.0/100.0 & 1 & 8.0 & 21.5 & 36.0 & 2000 \\
ADHD & DAT+BW & 100.0/100.0 & 73 & 108.0 & 141.0 & 215.0 & 635 \\
ADHD & TRI & 100.0/100.0 & 1 & 2.0 & 5.0 & 19.0 & 330 \\
ADHD & CLI & 100.0/100.0 & 2 & 2.0 & 5.0 & 9.0 & 49 \\
ADHD & RCLI & 95.0/98.4 & 3 & 5.0 & 12.0 & 45.0 & 622 \\
ADHD & DAT & 100.0/100.0 & 124 & 124.0 & 124.0 & 124.0 & 124 \\
\hline
ADHDM & EDG & 33.7/100.0 & 1 & 13.75 & 60.5 & 2000.0 & 2000 \\
ADHDM & DAT+BW & 100.0/100.0 & 71 & 193.0 & 372.0 & 606.0 & 1238 \\
ADHDM & TRI & 98.1/100.0 & 1 & 5.0 & 185.0 & 282.0 & 664 \\
ADHDM & CLI & 40.4/100.0 & 2 & 2.0 & 39.0 & 60.0 & 60 \\
ADHDM & RCLI & 60.6/100.0 & 3 & 8.0 & 307.0 & 548.0 & 632 \\
ADHDM & DAT & 100.0/100.0 & 124 & 124.0 & 124.0 & 124.0 & 124 \\
\hline
OHSU & EDG & 100.0/86.7 & 2 & 38.0 & 67.0 & 117.0 & 2000 \\
OHSU & DAT+BW & 100.0/100.0 & 40 & 100.0 & 149.0 & 196.0 & 889 \\
OHSU & TRI & 61.8/57.8 & 1 & 23.0 & 49.0 & 95.0 & 627 \\
OHSU & CLI & 52.9/86.7 & 2 & 29.0 & 60.0 & 82.0 & 97 \\
OHSU & DAT & 100.0/100.0 & 80 & 80.0 & 80.0 & 80.0 & 80 \\
\hline
PEK & EDG & 100.0/91.3 & 1 & 2.0 & 5.0 & 12.0 & 2000 \\
PEK & DAT+BW & 100.0/100.0 & 10 & 26.0 & 60.0 & 95.0 & 387 \\
PEK & TRI & 88.7/95.7 & 1 & 1.0 & 4.0 & 15.0 & 492 \\
PEK & CLI & 100.0/91.3 & 2 & 2.0 & 4.0 & 20.0 & 97 \\
PEK & DAT & 100.0/100.0 & 86 & 86.0 & 86.0 & 86.0 & 86 \\
\hline
KKI & EDG & 89.7/100.0 & 1 & 1.0 & 2.0 & 10.0 & 2000 \\
KKI & DAT+BW & 100.0/100.0 & 5 & 16.0 & 27.0 & 51.0 & 224 \\
KKI & TRI & 89.7/70.5 & 1 & 1 & 3.0 & 17.0 & 234 \\
KKI & CLI & 89.7/100.0 & 2 & 2.0 & 4.0 & 20.0 & 97 \\
KKI & DAT & 100.0/100.0 & 84 & 84.0 & 84.0 & 84.0 & 84 \\
  \bottomrule
	\end{tabular}
\end{table*}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Configuration of {\cli}}\ref{sec:settings}
\mynote[from=Carlo]{Do we want to keep it? To be updated and aligned with current notation.}{}
\Cref{tab:res} reports the performance of {\cli} in AUT-CS, for different parameter configurations.
It displays the flip Rrate $\mathsf{fr}$, and the percentile of number of iteraton $I$ and distance $d_{\%}$.
The configurations considered are the following:
\begin{itemize}
    \item Node Ranking Strategy $R$: $\mathsf{t}$ sorts the nodes based on the number of triangles, and $\mathsf{eg}$ based on the eigenvector centrality~\cite{10.5555/1809753};
    \item Sorting Strategy for $D$: $0$ means no sorting, $l_{+1}$ means the use of a vector that weights node in \Cref{alg:LS}, and $h_{-1}$ means the use of a vector that weights node in \Cref{alg:HS}.
\end{itemize}

We observe that the quartiles of the two distributions are similar across the configurations, whereas the flip rate $\mathsf{fr}$ shows an increase of $10\%$ between the two extreme settings. We register the following results:
\begin{itemize}
	\item The Node Sorting for Fill Search $D_n$ performs better with only the weights in the Empty Search $l_{+}$.
	\item $k$ shows not much difference in performance: a bit of budget but not too much.
	\item $NS$ the eigenvector centrality sorting $Eg$ reaches the best $\mathsf{fr}$.
\end{itemize}

\begin{table}[t]
    \centering
    \small
    \caption{Flip rate $\mathsf{fr}$, and quartiles of computation time $I$ and closeness $d_{\%}$, for different parameter configurations of {\cli}, in AUT-CS.}
    \label{tab:res}
    \begin{tabular}{c ccccc ccccc ccc}
	\toprule
	& \multicolumn{5}{c}{$I$} & \multicolumn{5}{c}{$d_{\%}$} & & &\\
	\cmidrule(lr){2-6} \cmidrule(lr){7-11}
		$\mathsf{fr}$ & 
		\textbf{Q0} & \textbf{Q1} & \textbf{Q2} & \textbf{Q3} & \textbf{Q4} & 
		\textbf{Q0} & \textbf{Q1} & \textbf{Q2} & \textbf{Q3} & \textbf{Q4} &
		\textbf{$D$} & \textbf{$k$} & \textbf{$R$} \\
		\midrule
		73.3 
		& 1 & 2 & 6 & 15 & 56 
		& 1.9 & 9.3 & 19.2 & 27.3 & 48.7 
		& \textbf{$0$} & 2 & $\mathsf{t}$\\
		68.3 
		& 1 & 2 & 8 & 15 & 58 
		& 1.9 & 9.3 & 19.7 & 29.9 & 55.8 
		& $l_{+1}$ & \textbf{4} & $\mathsf{t}$\\
		76.2 
		& 1 & 2 & 6 & 16 & 56 
		& 1.9 & 9.3 & 19.7 & 28.3 & 54.6 
		& $l_{+1}$ & 2 & $\mathsf{t}$\\
		78.2 
		& 1 & 2 & 7 & 18 & 56 
		& 1.9 & 10 & 20.1 & 32.8 & 53 
		& $l_{+1}$ & \textbf{0} & $\mathsf{t}$\\
		\textbf{79.2} 
		& 1 & \textbf{1} & \textbf{5} & 14 & 57 
		& 2.7 & \textbf{7.3} & 20.6 & 32 & 53.4 
		& $l_{+1}$ & 2 & \textbf{$\mathsf{eg}$}\\
		71.3 
		& 1 & 2 & 6 & 13 & 58 
		& 1.9 & 8.5 & 18.8 & \textbf{26.4} & 53 
		& \textbf{$l_{+1}$,$h_{-1}$} & 2 & $\mathsf{t}$\\
		\bottomrule
	\end{tabular}
\end{table}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The counterfactual graph can be visualized by coloring the edges in the symmetric difference with different colors, as shown in \ref{fig:local_1} (top).
This picture shows the brain connectome of a counterfactual explanation for a graph in ADHDM dataset in the class ``not used'', where the edges in $\{E \setminus E'\}$ (edges removed, for a total of $21$) are denoted in red, and the edges in $\{E' \setminus E\}$ (edges added, for a total of $16$) are denoted in blue.
Each node represents a voxel, and different node colors indicate different areas of the brain.

\begin{figure}[thb]
    \begin{minipage}[b]{\textwidth}
    \centering
    \includegraphics[width=\textwidth]{Figures/brains/legend.pdf}
   \end{minipage}
   \hfill
   \begin{minipage}[b]{0.49\textwidth}
    	\centering
    	 \includegraphics[width=\linewidth]{Figures/lzr_0_adhdm.pdf}
   \end{minipage}
   \begin{minipage}[b]{0.49\textwidth}
    	\centering
    	\includegraphics[width=\linewidth]{Figures/barplot_0.pdf}
   \end{minipage}
   % \begin{subfigure}[b]{\columnwidth}
   %  	\centering
   %  	\includegraphics[width=\linewidth]{Figures/heatmap.pdf}
   % \end{subfigure}
    \vspace{-4mm}
    \caption{Brain connectome of a counterfactual graph in the ``Marijuana use'' class in ADHDM (top), and summary of edges changed in each region of the brain (bottom).}
    \label{fig:local_1}
\end{figure}


The bar plot in \ref{fig:local_1} (bottom) shows which region of the brain the edges changed belong to.
In details, it reports the ratio of edges changed by region and by type of change (edges added $E^+$ and edges removed $E^-$).
This plot allow us to analyze which parts of the brain should be sparsified/densified to obtain a brain network classifiable in the ``Marijuana use'' class.
As we can see, we need to remove edges between the Frontal and Parietal Lobe, and add edges in the Posterior Fossa.

\begin{figure}[thb]
	\begin{minipage}[b]{0.49\textwidth}
    	\centering
    	 \includegraphics[width=\linewidth]{Figures/lzr_18_autcs.pdf}
   \end{minipage}
   \begin{minipage}[b]{0.49\textwidth}
    	\centering
    	\includegraphics[width=\linewidth]{Figures/barplot_18_autcs.pdf}
   \end{minipage}
	\vspace{-4mm}
	\caption{Brain connectome of a counterfactual graph in the TD class in AUT-CS (top), and summary of edges changed in each region of the brain (bottom).}
   \label{fig:local_2}
\end{figure}

\begin{figure}[thb]
    \begin{minipage}[b]{0.49\textwidth}
        \centering
        \includegraphics[width=\linewidth]{Figures/lzr_0_adhd.pdf}
   \end{minipage}
   \begin{minipage}[b]{0.49\textwidth}
    	\centering
    	\includegraphics[width=\linewidth]{Figures/barplot_0_adhd.pdf}
   \end{minipage}
   \vspace{-4mm}
   \caption{Brain connectome of a counterfactual graph in the TD class in ADHD (top), and summary of edges changed in each region of the brain (bottom).}
   \label{fig:local_3}
\end{figure}

\ref{fig:local_2} and \ref{fig:local_3} display the the brain connectome of counterfactual graphs in the TD class for a graph in AUT-CS (\ref{fig:local_2}) and in ADHD (\ref{fig:local_3}).
In the former, the symmetric difference with the original graph is 63 (32 edges removed and 31 added); while in the latter, the symmetric difference is 41 (21 edges removed and 20 added).

We can see that the brain with ASD has fewer connections in the Posterior Fossa than the brain with ADHD, as such region includes most of the edges added (resp. removed) to find the corresponding counterfactual graph.
Moreover, voxels in the Central Structures of the ADHD brain are more interconnected than those in a TD brain.


